Zero Resource Code-switched Speech Benchmark Using Speech Utterance Pairs For Multiple Spoken Languages

We introduce a new zero resource code-switched speech benchmark designed to directly assess the code-switching capabilities of self-supervised speech encoders. We showcase a baseline system of language modeling on discrete units to demonstrate how the code-switching abilities of speech encoders can be assessed in a zero-resource manner. Our experiments encompass a variety of well-known speech encoders, including Wav2vec 2.0, HuBERT, XLSR, etc. We examine the impact of pre-training languages and model size on benchmark performance. Notably, though our results demonstrate that speech encoders with multilingual pre-training, exemplified by XLSR, outperform monolingual variants (Wav2vec 2.0, HuBERT) in code-switching scenarios, there is still substantial room for improvement in their code-switching linguistic abilities.

==> figures/no_dedup.tex <==
\scalebox{1}{\begin{tikzpicture}
\begin{axis}[
    title={es-en},
    width=.5\textwidth,
    height=6cm,
    xlabel={$M$},
    ylabel={acc},
    %xmin=0.7, xmax=5.2,
    %ymin=25.0, ymax=40.0,
    %xtick={1,...,5},
    xtick={5, 10, 20, 50, 100},
    %xticklabels={5,10,20,50,100},
    %x tick label style={rotate=40,anchor=east},
    ytick={24, 26, 28, 30, 32, 34, 36, 38, 40},
    legend style={nodes={scale=0.8, transform shape}}, 
    legend pos=north east,
    ymajorgrids=true,
    grid style=dashed,
    label style={font=\small},
    tick label style={font=\small} 
]

\addplot[
    color=blue,
    mark=square,
    mark options={scale=0.5}
    ]
    coordinates {
        (0.3, 32.27)
        
        
        };
\addplot[
    color=black,
    mark=square,
    mark options={scale=0.5}
    ]
    coordinates {
        (0.3, 68.87)
        };
\addplot[
    color=red,
    mark=square,
    mark options={scale=0.5}
    ]
    coordinates {
        (1, 29.57)
        };
    \legend{$10$ min, $1$h}
    
\end{axis}
\end{tikzpicture}
}

==> tables/no_dedup.tex <==
\begin{table*}[ht]
\setlength\tabcolsep{4.5pt}
\renewcommand{\arraystretch}{1.0}
\centering
\begin{tabular}{lccccccc}
\toprule
           &           & km: 100 cluster        & Unit LM (roberta)       & quantize & es-en  & fr-en  & zh-en  \\
Speech Encoder         & \# param (B) & mono speech (hr)           & mono speech (hr)            & dedup        & test   & test   & test   \\
\midrule
\midrule
\multicolumn{8}{c}{Multilingual Speech Encoders}\\
\midrule
Whisper medium         &           & es, fr, zh, en 25 each & es, fr, zh, en 100 each & X            &        &        &        \\
XLSR-53 (53 lang)               & 0.3       & es, fr, zh, en 25 each & es, fr, zh, en 100 each & X            & 32.27 & 42.19 & 49.65 \\
XLS-R 0.3B  (128 lang)           & 0.3       & es, fr, zh, en 25 each & es, fr, zh, en 100 each & X            & 68.87 & 50.87 & 44.21 \\
XLS-R 1B     (128 lang)          & 1         & es, fr, zh, en 25 each & es, fr, zh, en 100 each & X            & 29.57 & 35.30  & 41.91 \\
mHuBERT                & 0.09      & es, fr, en 33 each     & es, fr, en 133 each     & X            & 26.78 & 26.57 & 41.06 \\
\midrule
\midrule
\multicolumn{8}{c}{Monolingual Speech Encoders}\\
\midrule
Wav2vec2 LARGE (ll60k) & 0.3       & en 100                 & en 400                  & X            & 12.89 & 26.47 & 38.98 \\
HuBERT X-LARGE (ll60k)        & 1         & en 100                 & en 400                  & X            & 14.26 & 18.81 & 40.30 \\
HuBERT Base (LS960)           & 0.09      & en 100                 & en 400                  & X            & 10.95 & 16.82 & 40.68 \\
\midrule
\midrule
random                 & -         & random                 & random                  & -            & 23.63 & 32.11 & 37.47\\
\midrule
text-based roberta topline &  - & - & - & - & & & \\
text-based XGLM topline &  - & - & - & - & 90.91 &	88.38 & 92.03\\
\bottomrule
\end{tabular}
\caption{}
\label{tab:no_dedup}
\end{table*}
